Robust Out-of-distribution Detection for Neural Networks

Detecting out-of-distribution (OOD) inputs is critical for safely deploying deep learning models in the real world. Existing approaches for detecting OOD examples work well when evaluated on benign in-distribution and OOD samples. However, in this paper, we show that existing detection mechanisms can be extremely brittle when evaluating on in-distribution and OOD inputs with minimal adversarial perturbations which don't change their semantics. Formally, we extensively study the problem of Robust Out-of-Distribution Detection on common OOD detection approaches, and show that state-of-the-art OOD detectors can be easily fooled by adding small perturbations to the in-distribution and OOD inputs. To counteract these threats, we propose an effective algorithm called ALOE, which performs robust training by exposing the model to both adversarially crafted inlier and outlier examples. Our method can be flexibly combined with, and render existing methods robust. On common benchmark datasets, we show that ALOE substantially improves the robustness of state-of-the-art OOD detection, with 58.4% AUROC improvement on CIFAR-10 and 46.59% improvement on CIFAR-100.

==> analysis.tex <==
%\paragraph{Why unlabeled data can help?}
%\yingyu{TODO: use Gaussian to show the decrease of sample complexity when $U_X$ is used}
%
%\paragraph{Why generalize to unseen outlier distributions?}

The interesting questions related to our method are: {\bf (1)} why unlabeled auxiliary data from $U_X$ helps? {\bf (2)} why the robustness of the detector $G$ on $U_X$ generalizes to a different distribution $Q_X$? 
%An interesting observation is that even when the OOD training data distribution $U_X$ is different from the OOD test data distribution $Q_X$, the trained detector still achieves great OOD detection performance on $Q_X$. When will a detector trained on data from $P_X$ and $U_X$ generalize well to test data from $P_X$ and $Q_X$? 

To get some intuition for these questions, we adopt the domain adaption framework~\citep{ben2010theory}. Recall that in domain adaptation there are two domains $\bm{s}, \bm{t}$, each being a distribution over the input space $\mathcal{X}$ and label space $\{0,1\}$. A classifier is trained on $\bm{s}$ then applied on $\bm{t}$. We view our OOD detection problem as classification, where the source domain $\bm{s}$ is $P_X$ with labels $1$ and $U_X$ with labels $0$, and the target domain $\bm{t}$ is $P_X$ with labels $1$ and $Q_X$ with label $0$. 

Denote the loss of detector $G$ on point $(x,y)$ as:
$$
L(G, x, y; \Omega) := \max_{\delta \in \Omega(x)}\mathbb{I}[G(x+\delta) \neq y].
$$ 
Denote the loss of $G$ in the source domain as:
\begin{align*}
R^{\bm{s}}(G) & := \frac{1}{2}\mathbb{E}_{x \sim P_X, y=1} L(G, x, y; \Omega)  + \frac{1}{2}\mathbb{E}_{x \sim U_X, y=0} L(G, x, y; \Omega)
\end{align*}
and similarly define the loss $R^{\bm{t}}(G)$ of $G$ in the target domain. Following~\cite{ben2010theory}, define (a variant) of the divergence of $Q_X$ and $U_X$ w.r.t.\ the hypothesis class $\mathcal{G}$ as
\begin{align*}
d_{\mathcal{G}}(Q_X, U_X) = \sup_{G, G' \in \mathcal{G}} v(G, G'; Q_X) - v(G, G'; U_X) 
\end{align*}
where 
\begin{align*}
v(G, G'; D) = \mathbb{E}_{x \sim D, y=0} (L_{\Omega}(G, x, y) - L_{\Omega}(G', x, y))
\end{align*}
is the loss difference of $G$ and $G'$ on distribution $D$. 
The divergence upper bounds the change of the hypothesis loss difference between $Q_X$ and $U_X$. If it is small, then for any $G, G' \in  \mathcal{G}$ where $G$ has a smaller risk than $G'$ in $U_X$, we know that $G$ will also have a smaller (or not too larger) risk than $G'$ in $Q_X$. That is, if the divergence is small, then the ranking of the hypotheses w.r.t.\ the loss is roughly the same in both distributions. This \emph{rank-preserving} property thus makes sure that a good hypothesis learned in $U_X$ will also be good for $Q_X$. 

Now we show that, if $d_{\mathcal{G}}(Q_X, U_X)$ is small (i.e., $Q_X$ and $U_X$ are aligned w.r.t.\ the class $\mathcal{G}$), then a detector $G$ with small loss in the source domain will also have small loss in the target domain. 
\begin{thm} \label{thm:unlabel}
For any $G \in \mathcal{G}$, 
\begin{align*}
R^{\bm{t}}(G) 
& \le \inf_{G^* \in \mathcal{G}} R^{\bm{t}}(G^*) + R^{\bm{s}}(G) + \frac{1}{2} d_{\mathcal{G}}(Q_X, U_X).
\end{align*}
\end{thm}
\begin{proof}
See the Appendix \ref{sec:proof-theorem-1}. 
\end{proof}

The test error of the detector is bounded by three terms: the best error, the error on the training distributions, and the divergence between $Q_X$ and $U_X$. Assuming that there exists a ground-truth detector with a small test error, and that the optimization can lead to a small training error, the test error is then characterized by the divergence. So in this case, as long as the rankings of the hypotheses (according to the error) on $Q_X$ and $U_X$ are similar, detectors learned on $U_X$ can generalize to $Q_X$. 

\paragraph{An illustration example.} 
In this example, the in-distribution $P_X$ is uniform over the disk around the origin in $\mathbb{R}^2$ with radius $1$, $U_X$ is uniform over the disk around $(0,3)$ with radius $1$, and $Q_X$ is uniform over the disk around $(3,0)$ with radius $1$. Assume the adversary budget is $\epsilon=0.1$, i.e., $\Omega=\{\|\delta\|_2 \le 0.1\}$. The hypothesis class for the detector contains all functions of the form $G_r(x) = \mathbb{I}[\|x\|_2 \ge r]$ with parameter $r$. See Figure~\ref{fig:illustration-example}.

\begin{figure*}[t!]
	\centering
	\includegraphics[width=0.4\linewidth]{figures/illustration-example.pdf}
	\hspace{1cm}
	\caption{\small An illustration example to explain why $U_X$ helps to get a good detector $G_r$.  With $U_X$, we can prune away hypotheses $G_r$ for any $r \geq 1.9$. Thus, the resulting detector $G_r$ can detect OOD samples from $Q_X$ successfully and robustly.}
	\label{fig:illustration-example}
\end{figure*}

The example first shows the effect of the unlabeled data: $U_X$ helps to prune away hypotheses $G_r$ for any $r\ge 1.9$. Furthermore, it also shows how learning over $U_X$ can generalize to $Q_X$. 
Although $Q_X$ and $U_X$ have non-overlapping supports, $U_X$ help to calibrate the error of the hypotheses so that any good detector trained on $P_X$ and $U_X$ can be used for distinguishing $P_X$ and $Q_X$. Formally, the $d_{\mathcal{G}}$ is small in Theorem~\ref{thm:unlabel}.

The analysis also shows the importance of training on \emph{perturbed} instances from the unlabeled data $U_X$. Not using perturbation is equivalent to using $\Omega=\{\bm{0}\}$. In this case, the analysis shows that it only guarantees the error on \emph{unperturbed} instances from $Q_X$, even if $Q_X$ and $U_X$ has small divergence and the optimization gives small training error. 
